Membership Inference Attack Using Self Influence Functions

Member inference (MI) attacks aim to determine if a specific data sample was used to train a machine learning model. Thus, MI is a major privacy threat to models trained on private sensitive data, such as medical records. In MI attacks one may consider the black-box settings, where the model's parameters and activations are hidden from the adversary, or the white-box case where they are available to the attacker. In this work, we focus on the latter and present a novel MI attack for it that employs influence functions, or more specifically the samples' self-influence scores, to perform the MI prediction. We evaluate our attack on CIFAR-10, CIFAR-100, and Tiny ImageNet datasets, using versatile architectures such as AlexNet, ResNet, and DenseNet. Our attack method achieves new state-of-the-art results for both training with and without data augmentations. Code is available at https://github.com/giladcohen/sif_mi_attack.

==> sec/7_checklist.tex <==
\section*{Checklist}
%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%
\begin{enumerate}
\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:conclusions}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section~\ref{sec:conclusions}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The complete code can be found in the supp. mat.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{The target models' hyperparameters, data split, and training procedure is discussed in Section~\ref{sec:target_model}. The attack model's data split is discussed in Section~\ref{sec:attack_model_training_and_evaluation}. The attack model's pseudo code and the algorithm that chooses its two thresholds is provided in the supp. mat.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report error as standard deviation in the ablation experiment (see Figure~\ref{fig:ablation}), however other experiments were reported with only one seed due to long run time.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We report fitting and inference time for our methods and baselines in Section~\ref{sec:computational_cost}. Our CPU and GPU apparatus is listed in the supp. mat.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{The CIFAR-10, CIFAR-100, and Tiny ImageNet datasets have been cited.}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


==> supp_sec/0_metadata.tex <==
\title{Membership Inference Attack Using\\ Self Influence Functions\\ (Supplementary Material)}


% The \author macro works with any number of authors. There are two commands
% used to separate the names and addresses of multiple authors: \And and \AND.
%
% Using \And between authors leaves it to LaTeX to determine where to break the
% lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4
% authors names on the first line, and the last on the second line, try using
% \AND instead of \And before the third author name.

\author{%
  Anonymous Author(s) \\
}


==> supp_sec/intro.tex <==
The supplementary material is organized as follows:
\begin{itemize}
    
\item Appendix~\ref{supp_sec:sif_algorithm} provides pseudo codes to outline the fitting and inference of our membership inference (MI) attack model.

\item Appendix~\ref{supp_sec:efficient_sif_calculation} explains in detail how the self-influence measure was approximated for SIF and adaSIF.

\item Appendix~\ref{supp_sec:hardware_setup} lists the hardware (CPUs \& GPUs) we used for training the target models and for fitting/evaluating our attack models.

\item Appendix~\ref{supp_sec:accuracy_of_target_models} reports the train/test accuracies for all the target models.

\item Appendix~\ref{supp_sec:comparison_of_mi_attacks} compares our MI attack to baselines for target models trained on AlexNet and DenseNet architectures.

\item Appendix~\ref{supp_sec:precision_and_recall} reports the precision and recall metrics on members and non-members, for our attack model and baselines.

\item Appendix~\ref{supp_sec:naive_sif_ensemble} advocates the use of our proposed adaSIF over a naive SIF ensemble.

\item Appendix~\ref{supp_sec:comparison_of_mi_attacks_with_data_augmentation} compares the attack performance of adaSIF to baselines, for target models trained with data augmentations on AlexNet and DenseNet.

\item Appendix~\ref{supp_sec:comparison_to_a_white_box_attack} compares our MI attack methods to an additional white-box attack.

\end{itemize}
